CSLP-AE: A Contrastive Split-Latent Permutation Autoencoder Framework for Zero-Shot Electroencephalography Signal Conversion

Electroencephalography (EEG) is a prominent non-invasive neuroimaging technique providing insights into brain function. Unfortunately, EEG data exhibit a high degree of noise and variability across subjects hampering generalizable signal extraction. Therefore, a key aim in EEG analysis is to extract the underlying neural activation (content) as well as to account for the individual subject variability (style). We hypothesize that the ability to convert EEG signals between tasks and subjects requires the extraction of latent representations accounting for content and style. Inspired by recent advancements in voice conversion technologies, we propose a novel contrastive split-latent permutation autoencoder (CSLP-AE) framework that directly optimizes for EEG conversion. Importantly, the latent representations are guided using contrastive learning to promote the latent splits to explicitly represent subject (style) and task (content). We contrast CSLP-AE to conventional supervised, unsupervised (AE), and self-supervised (contrastive learning) training and find that the proposed approach provides favorable generalizable characterizations of subject and task. Importantly, the procedure also enables zero-shot conversion between unseen subjects. While the present work only considers conversion of EEG, the proposed CSLP-AE provides a general framework for signal conversion and extraction of content (task activation) and style (subject variability) components of general interest for the modeling and analysis of biological signals.

==> 5discussion_old_do_not_edit.tex <==
%\section{Discussion}
%\label{sec:discussion}

The addition of the split-latent permutation loss to the contrastive learning model had little effect on the topology of the task latent space (see \cref{fig:tsne}),
and had some effect on the topology of the subject latent space. However, both measures of disentanglement, subject and task classification accuracy, did see an increase in performance from the addition of the split-latent permutation loss (see \cref{result-table}).
It also provided a significant increase in performance on the (D.s./S.t.) and (S.s./D.t.) ERP conversion tasks (see \cref{result-table}).
The improvement in conversion performance can be attributed solely to the capabilities of the decoder and the information flow within it, specifically the implicitly learned permutation-invariance, as the topology of the latent space did not undergo significant changes due to the addition.

%\subsection{Structural encoding}
The $t$-SNE plots and the results of the conversion on different subjects/different tasks show a tendency.
The latent-permutation trained latent spaces are topologically similar (or to some degree even identical) which raises one point:
\emph{structural encoding}; depending on the method or loss, the auto-encoder might only learn a structural encoding.

The different ERP conversion methods described in \cref{sec:experiments} are increasingly more difficult to convert from. 
(S.s./S.t.) allows structural information through both latent spaces, while (D.s./S.t.) and (S.s./D.t.) only allow structural information through one latent space.
(D.s./D.t.) is really hard requiring conversion with no retainment of any structural information whatsoever for the decoder to rely on, i.e. conversion must be done using only abstract subject and task embeddings, and structure must arise from these.

Models trained with latent-permutation learns this structural encoding in the latent spaces since the decoder can rely on at least one of the latent spaces in the latent-swap procedure (\cref{fig:latentpermutation}) to provide the structural information of the EEG signal.
This structural information, although indistinguishable in different latent spaces, coincidentally is highly correlated with both subject and task content of the signal. This structural encoding is most notable in the SLP-AE latent space as shown in \cref{fig:tsne} allowing the classifier to perform well on all classification tasks. The SLP-AE model, however, obtains worse performance on subject classification compared to the other deep learning models - but interestingly enough, it has identical performance of subject and task classification as applied in both latent spaces (S.acc\%$\approx$S$\vdash$T.acc\% and T.acc\%$\approx$T$\vdash$S.acc\% for SLP-AE in \cref{result-table}).

Contrastive learning in the latent space itself has nothing to do with decoding the structure of the data for reconstruction. The encoder is simply trained to learn an embedding of the subject and task content of the signal. The decoder must, therefore, do the heavy work of extracting this structural information itself. This exposes a property which is applicable to the latent-permutation method but not contrastive learning. When the stand-alone latent-permutation method is used (SLP-AE), the decoder is allowed a reliability in the latent spaces.
A lot of the EEG signal is structural information, therefore, 
there might be more to gain from minimizing the permutation-invariance to structural information rather than encoding the subject and task content directly.
It might be easier for the decoder to simply learn a permutation-invariant structural encoding of the signal in both latent spaces,
which allows the decoder to rely on this information irrespective of the permutation or swap - since only one latent space (see \cref{fig:latentpermutation}) is swapped at a time. Thus, The latent-permutation only trained model (SLP-AE) does not learn explicitly disentangled representations of the subject and task content of the signal,
but rather a duplicated latent space permutation-invariant structural encoding which is highly correlated with both subject and task content of the signal.
This interestingly is also the goal of the standard autoencoder. The latent-permutation method allows the model to learn an encoding explicitly in the latent space instead of implicitly in the encoder/decoder architectures.
This might be a powerful tool since it further constricts the bottleneck in the auto-encoder sense, although at the cost of suboptimally encoding identical latent spaces. This can be, and is, remedied by using both contrastive learning and latent-permutation in conjunction.


Having completely disentangled latent spaces is a local minimum in the latent-permutation method and allows for the ideal swap in \cref{fig:latentpermutation}(a). The CSLP-AE model is able to keep the latent spaces disentangled while also providing the structural encoding information required for the conversion method to work.
This is evident from \cref{result-table} which shows that the stand-alone latent-permutation model (SLP-AE) achieves about half ($\approx51.7\%$) the MSE error of the C-AE model on the ERP conversion tasks using samples from different tasks or subjects (D.s/S.t. and S.s./D.t.), and the CSLP-AE model retains this performance.
The latent-permutation method described in this paper is then proposed as a replacement for the standard auto-encoder reconstruction loss to be used in conjunction with contrastive learning to provide a disentangled latent space which also allows for the structural encoding information to flow through the latent spaces and ease zero-shot conversion.

The latent-permutation method does not increase performance on the (D.s./D.t.) conversion task. Arguably the difference in performance between the stand-alone latent-permutation and contrastive learning methods (on D.s/S.t. and S.s./D.t.) is due to this structural encoding property. An analysis is provided in the supplementary material providing a generalization of the latent-permutation method onto different subject/different task conversion to circumvent the structural encoding reliability. %MISSING SUPPLEMENTARY

Further research could explore different avenues for keeping structural information while also disentangling subject and task latents,
or providing a source for this structural encoding using generative methods or distributional power to generate structure, e.g. through the use of a VAEs. \citep{kingma2013auto}


%Show the three main model TSNEs and compare structuredness
%Structuement between LP and QP: LP allows structure information to flow through latents, while QP does not (whole new data) <-- this structure may be what causes the LP to descend to the local minima where both spaces encode the same information (which is evidently the structural information - and which is definitely correlated to both subject and task ebmeddings (see this as noise which provides the given structure of the sample))
%^^ Also there might be more to gain from minimizing the permutation-invariance to structure information rather than encoding the subject and task content directly.
%With QP this is alleviated since it can not rely on structure information anymore. However, this also disintegrates the conversion itself, since it now has no "easy" path to encode structural information.
%A third splti which is independent of any loss which can provide this structure data might be relevant?
%ERP conversion loss: different degrees of separability from structured information; with Ds/Dt the model is not even able to keep information about general structurality.
%The non-specialization of the latent space may be due to that it is easier to minimize the structural MSE loss and provide such structure in both latent spaces, which is definitely correlated with both subject and task content but does not itself provide the desired disentanglement. Therefore, stems the need for the use of the contrastive learning method in supplement to the latent permutation loss.
%Partition of each latent space into both subject and task embeddings: bypasses both permutation-invariance, minimizes structural MSE loss and does not explicitly disentangle instead hiearchically/partitionally encodes both subject and task embeddings in both spaces.
%D.s/D.t is really hard requiring no retainment of any structural information whatsoever.
%explroe avenues for keeping structural info while also disentangling subject and task content information - or providing distributional power through VAE for it to generate structure in the data based on latent distribution

\section{Conclusion, Limitations, and Broader Impact}
In this paper, a novel split-latent permutation framework was introduced for disentangling subject and task content in EEG signals and enabling single-trial zero-shot conversion. By combining auto-encoders and contrastive learning, superior results were achieved compared to standard deep learning methods on the standardized ERP Core dataset. The experimental results demonstrated a significant 51.7\% improvement in ERP conversion loss on unseen to unseen subject conversions. The method also achieved high single-trial subject classification accuracy (80.32±0.28\%) and single-trial task classification accuracy (51.38±0.21\%) on unseen subjects.

The findings of this paper are limited to the single dataset used for the experiments. However standardized the dataset is, it is still a single dataset with similar measurement conditions for all subjects. Therefore, the results of this paper may not generalize to other datasets with different measurement conditions.  Similarly, due to the nature of the contrastive learning method, other datasets require standard EEG measurements over several different tasks to be used for training. The ERP Core dataset \citep{kappenman2021erp} used here is an effort to standardize ERP measurements with more data to come in the future from other laboratories which might alleviate this limitation. The tasks used in the experiments are all seen during training. This limits the scope of the results to the seen tasks and no conclusions can be drawn about the generalization of the model to unseen tasks.

Zero-shot conversion of EEG signals, similar to other deep fake methods, can be used for malicious purposes. Methods discussed in this paper intrude on one of the most sacred places yet to be exploited and confused by technology: the human mind.
Malicious use of this technology includes the ability to decode thoughts and intentions from EEG signals, and the ability to create fake EEG signals to confuse verification systems using EEG signals as a biometric identifier.
Care must be taken when developing and deploying such technology to ensure that it is not used for malicious purposes. However, it can also be used to improve the quality of life for people with and without disabilities. It provides a base for generalizing EEG signal representations across subjects and tasks, which can be used to improve the performance of EEG-based BCI systems, especially on a single-trial level as attestable by the results in \cref{result-table}. Similarly, it provides a base for analyzing EEG signals from a different perspective. One such perspective is to analyze EEG signals of a healthy person by their converted signals to that of a sick or disabled person, or by predicting their reaction to a certain stimulus. However, care must be taken when analyzing results from zero-shot conversions due to their inaccurate predictive nature.% - they may be misleading.
%Use of subject latent as biological signature
%Conversion allows to see EEG signals from the perspective of a *sick* person.
%Discuss here what this technology improves and its applications.

%\section{Conclusion}
%In this paper, a novel split-latent permutation framework was introduced for disentangling subject and task content in EEG signals and enabling single-trial zero-shot conversion.
%By combining auto-encoders and contrastive learning, superior results were achieved compared to standard deep learning methods on the standardized ERP Core dataset.
%The experimental results demonstrated a significant 51.7\% improvement in ERP conversion loss on unseen to unseen subject conversions. The method also achieved high single-trial subject classification accuracy (80.32±0.28\%) and single-trial task classification accuracy (51.38±0.21\%) on unseen subjects.

